Bandit algorithms: Letting go of logarithmic regret for statistical robustness

We study regret minimization in a stochastic multi-armed bandit setting and establish a fundamental trade-off between the regret suffered under an algorithm, and its statistical robustness. Considering broad classes of underlying arms' distributions, we show that bandit learning algorithms with logarithmic regret are always inconsistent and that consistent learning algorithms always suffer a super-logarithmic regret. This result highlights the inevitable statistical fragility of all `logarithmic regret' bandit algorithms available in the literature---for instance, if a UCB algorithm designed for $\sigma$-subGaussian distributions is used in a subGaussian setting with a mismatched variance parameter, the learning performance could be inconsistent. Next, we show a positive result: statistically robust and consistent learning performance is attainable if we allow the regret to be slightly worse than logarithmic. Specifically, we propose three classes of distribution oblivious algorithms that achieve an asymptotic regret that is arbitrarily close to logarithmic.

==> sections/upper_bounds-old.tex <==

\section{Near-optimal oblivious algorithms}
\label{upper-bounds}
After establishing the impossibility of the existence of an oblivious algorithm over the distributions of interest, we propose near-optimal algorithms. In an oblivious setting, the parameters of the underlying reward distribution cannot be used as an input to the algorithm. Devising a suitable oblivious concentration inequality is crucial in proving a theoretical upper bound to an algorithm. To take into account the effect of an unknown parameter, we introduce a suitable monotonic function which varies with the number of rounds. We make the function increasing or decreasing depending on the nature of the concentration inequality we intend to work with. The choices of the function and its monotonicity ensures that the inequality is guaranteed for all $t>t_{min}$, where $t_{min}$ depends on the parameter of the underlying distribution and the choice of the function. We can therefore assume that the inequalities are true in limiting sense. Hence, the cumulative regret upper bound is also valid for asymptotic cases. For different choices of the function, we get different values of $t_{min}$. We will also see that there is a tradeoff between the value of $t_{min}$ and the asymptotic regret bound. If we are interested in lowering the $t_{min}$ we get a worse regret bound. Similarly, choosing the functions so that the bound is arbitrary close to being logarithmic results in a very high value of $t_{min}$. The algorithms we propose for the classes $\{\B, \SG,\G\}$ are any-time algorithms, that is, the algorithm does not require the knowledge of horizon. We propose another fixed-horizon algorithm for $\{\G\}$ which, as we will see, has a slightly better regret bound than the corresponding any-time algorithm (\ashutosh{asymptotic is same but $t_0$ is less for MoM because of it being central moment}).
% We denote this algorithm as $\pi_t$ .We also propose a fixed horizon algorithm $\pi_T$ for $\{\G\}$ which, as we shall see, has slightly better regret bound than the any-time algorithm $\pi_t$.

All the proposed algorithms are structurally similar to the Upper Confidence Bound (UCB) algorithm where we have a mean estimator and a confidence width. We define $\U(i, u, t)$ as the upper confidence bound of $i^{th}$ arm after being chosen $u$ times in $t$ rounds. Using a similar notation, we define $\hat{\mu}(i, u, t)$ as the mean estimator and  $\W(u, t)$ as the confidence width. Consequently, $\U(i, u, t) = \hat{\mu}(i, u, t) + \W(u, t)$. Note that the confidence width does not depend on either the reward distribution or the sampled value, thus being independent of arm index $i$. 
%Following the algorithm, we present regret bound for $\pi_t$.


For different class of oblivious distributions out of $\{\B, \SG,\G\}$, we get different confidence width $\W$. The choice of $\W$ depends on the concentration inequality to be employed. $\W$ is chosen so that the deviation of empirical mean from the true mean lies within $\W$ with a high probability. $\hat{\mu}$ is the mean estimator which is simply the empirical average for $\{\B,\SG\}$ and Truncated Empirical Estimator (TEA) for $\{\G\}$. We denote the three algorithms as $\pi_{\B}$, $\pi_{\SG}$ and $\pi_{\G_{TEA}}$ respectively. Finally, the fixed-horizon algorithm for $\{\G\}$ uses Median of Means (MoM) estimator for $\hat{\mu}$. We denote this algorithm by $\pi_{\G_{MoM}}$. Algorithm \ref{any-time-version} provides a pseudo-code for $\pi_{\B}$, $\pi_{\SG}$ and $\pi_{\G_{TEA}}$. The proves of the regret bound for the three class of distributions are similar to each other and hence we prove a rather generic Theorem \ref{general-upper-bound-thm} which states an expression for $\mathbb{E}[T_i(n)]$, that is, the expected number of times a sub-optimal arm is chosen.

\alternate{
\begin{theorem}
(Regret upper bound for algorithm \ref{robust-light-UCB-algo}) For all bandit instance $\nu \in \M^k$ where ${\M \in \{\B,\SG,\SE\}}$, and for all increasing function $f:\mathbb{N} \rightarrow \mathbb{R}$, the total cumulative regret till $t$ rounds of algorithm satisfies
$$ R_t(\pi_{RL-UCB}, \nu) \leq \sum_{j:\Delta_j>0} \left( 3\Delta_j + 16f(t)^2 \frac{\log(t)}{\Delta_j} \right) $$
\end{theorem}
}


%\begin{theorem}
%\label{general-upper-bound-thm} Consider algorithms $\pi_{\B}$, $\pi_{\SG}$ and $\pi_{\G_{TEA}}$. If $|\hat{\mu}(i, u, n) - \mu_{\{i,u,n\}}| > \W(u, n)$ with a probability less than $n^{-2}$ for given arm $i$, any $u>0$ and $n>t_{min}$, then we have
%\begin{align*}
%    \mathbb{E}[T_i(n)] &\leq u_i + 2 
%\end{align*}
%where $u_i$ is the minimum $u$ for which $\Delta_i > 2\W(u, n)$
%\end{theorem}

\begin{theorem}
\label{general-upper-bound-thm}
    Consider algorithms $\pi_{\B}$, $\pi_{\SG}$ and $\pi_{\G_{TEA}}$. Take a monotonically increasing function $f:\mathbb{N}\rightarrow \mathbb{R}$ and a monotonically decreasing function $g:\mathbb{N}\rightarrow \mathbb{R}^{+}$. We make the following choices for mean estimator $\hat{\mu}(i, u, t)$ and width $\W(u, t)$.
    \begin{align*}
        \pi_{\B}: \quad \hat{\mu}(i, u, t) = \sum_{j=1}^{u} X_j, \quad \W(u, t) = f(t)\sqrt{\frac{2\log(t)}{u}}
    \end{align*}
    \begin{align*}
        \pi_{\SG}: \quad \hat{\mu}(i, u, t) = \sum_{j=1}^{u} X_j, \quad \W(u, t) = f(t)\sqrt{\frac{8\log(t)}{u}}
    \end{align*}
    \begin{align*}
        \pi_{\G_{TEA}}: \quad \hat{\mu}(i, u, t) = \frac{1}{u} \sum_{i=j}^{u} X_j \mathbbm{1}_{\left\{|X_j|\leq \left( \frac{uf(t)}{4\log(t)} \right)^{\frac{1}{1+g(t)}} \right\}}, \W(u, t) = 4 f(t)^{\frac{1}{1+g(t)}} \left( \frac{\log(2t^{4})}{u} \right)^{\frac{g(t)}{1+g(t)}}
    \end{align*}
    \begin{align*}
        \alternate{\pi_{\G_{TEA}}: \quad \hat{\mu}(i, u, t) = \frac{1}{u} \sum_{i=j}^{u} X_j \mathbbm{1}_{\left\{|X_j|\leq f(t) \right\}}, \quad \W(u, t) = \frac{1}{\log(f(t))} + f(t) \frac{\log(2t^4)}{u}}
    \end{align*}
The following properties holds true for class of distribution $\{\B, \SG,\G\}$:
\begin{enumerate}
    \item There exists $t_{min}$ such that for all $t>t_{min}$, $\mathbb{P}\left( |\hat{\mu}(i, u, t) - \mu_{\{i,u,t\}}| \geq \W(u, t) \right) \leq t^{-4}$
    \item $\mathbb{E}[T_i(t)] \leq u_i + 2$ where $u_i$ is the minimum $u$ satisfying $\Delta_i \geq 2\W(u, t)$
\end{enumerate}
%    Suppose that
%    \begin{align*}
%        \sum_{s=1}^{t} \mathbb{P}(|\hat{\mu}(i, u, s) - \mu_{\{i,u,t\}}| \geq \W(u, s)) \leq \sum_{s=1}
%    \end{align*}
\end{theorem}

Property 1 of theorem \ref{general-upper-bound-thm} uses appropriate concentration inequalities for the three classes of distributions $\{\B, \SG,\G\}$. The choices of inequality and functions $f$ and $g$ ensures that the inequalities are valid for all $t>t_{min}$. We justify the choices of $\hat{\mu}(i, u, t)$ and $\W(u, t)$ in the next subsections. We use property 1 in proving property 2. Property 2 proposes a generic upper bound for all the three classes of algorithms. We will see that in all the cases the asymptotic regret bound can be made arbitrary close to logarithmic using suitable choices of $f$ and $g$.

%Since the concentration inequality we state are true only for $n>t_{min}$, the above expression is also true only for $n>t_{min}$. Now, we state suitable concentration inequality for $\{$\B$,\text{ } $\SG$,\text{ } $\G$\}$ and obtain a corresponding confidence width $\W$ in the next subsections.

%In the proof of the above theorem, we add $t^{-4}$ probability event from $t=u_i$ to $n$ and observe that the sum is upper bounded by a constant. However, we see that $|\hat{\mu}(i, u, t) - \mu_{\{i,u,t\}}| > \W(u, t)$ is a low probability event only for $t>t_{min}$. We also observe that as $n$ increases, $u_i$ will also increase but $t_{min}$ is constant with respect to the number of rounds. Hence a large value of $n$ ensures that we are indeed summing up the low probability events.

\begin{algorithm}[t]
  \caption{Robust Light RL-UCB ($\pi_{RL-UCB}$)}
  \label{robust-light-UCB-algo}
   \textbf{Input} $k$ arms, increasing function $f:\mathbb{N} \rightarrow \mathbb{R}$
  \begin{algorithmic}
    %\Statex \Comment { \%comment: servers[] contains the index of servers whose         data rate are sorted in descending order\%}
    %\Procedure UCB Algorithm
    %\State servers[]= index(of all servers) 
    % \State serverIndex[]=servers[0..K]
    % \State linearlyIndependentServerIndex[]=0
    % \State $[Z] \leftarrow 0$
    \For  {$t=1$ to $k$}
    \State pull arm with index $i = t-1$ and observe reward $r$
    \State Update $\hat{\mu}(i, u_i) \leftarrow r$, $u_i \leftarrow 1$
%    \Statex\Comment{ \%comment: find the equation corresponding the serverIndex        from the mapping at the File Server\%} 
%    \State        $eqn= equation(serverIndex[i])$ 
 %   \Statex\Comment{ \%comment: try insert equation into Z using OFG\%} 
    \EndFor 
    \For { $t=k+1, k+2, \dots$ } 
%    \Statex\Comment{\%comment: remove all the server index which were not inserted in Z\%}  
%	\State Calculate $\U(i, u, t) = \hat{\mu}(i, u, t) + \W(u, t)$
    \State Calculate the upper confidence bound as $$\U(i, u_i, t) = \hat{\mu}(i, u_i) + \underbrace{f(t) \sqrt{\frac{4\log(t)}{u_i}}}_{\W(u_i, t)} $$
	\State pull arm $i$ maximizing $\U(i, u_i, t)$ and observe reward $r$
	\State Update empirical average $\hat{\mu}(i, u, t)$ and $u\leftarrow u+1$
 %   \State pull $a_i = \underset{i}{\mathrm{argmin}}\text{ } \hat{\mu_{i}} + f(t) \sqrt{\frac{2\log(t)}{u_i}}$ and observe reward $r$
%    \State $\hat{\mu_t} \leftarrow \frac{\hat{\mu_t}u_i + r}{u_i + 1}$ \text{(Empirical mean update) }
%    \State $u_i \leftarrow u_i + 1$
    %temp[]=serverIndex[]-linearlyIndependentServerIndex 
    \EndFor  
    %\EndProcedure
  \end{algorithmic}
\end{algorithm}

\subsection{Confidence width $\W$, mean estimator $\hat{\mu}$ and regret $R_t(\pi_{\B})$ for $\B$}
The basic idea to obtain a concentration bound on $\B$ is to first obtain a similar concentration bound on $\B([a, b])$ and then replace the parameters $\{a, b\}$ with a suitable oblivious parameter. Hoeffding Inequality \ashutosh{(cite)} is a standard concentration inequality involving the mean of bounded random variables. We introduce a monotonically increasing function $f:\mathbb{N}\rightarrow\mathbb{R}$ in the confidence width $\W$. As a result of this, we get a term $\frac{f(t)}{(b-a)}$ in the concentration inequality that we use. Now from the instant $f(t) > (b-a)$, the inequality remains valid and we thus obtain an oblivious concentration inequality. Consequently $t_{min} = f^{-1}(b-a)$. We state the inequality that is used to obtain the width $\W$.

\begin{lemma}
\label{bounded-conc-inequality}
    Consider random variables $X_1, X_2, \dots, X_u \sim \B$ with mean $\mu$. For sufficiently large $t$, with a probability less than $\delta$, we have
    \begin{align*}
        \mu - \hat{\mu} \geq f(t)\sqrt{\frac{\log(\frac{1}{\delta})}{2u}} \leq \delta \qquad \text{where} \qquad \hat{\mu} = \frac{1}{u} \sum_{j=1}^{u} X_j
    \end{align*}
\end{lemma}
We choose $\delta=t^{-4}$ in Theorem \ref{general-upper-bound-thm}.
%Finally, Theorem \ref{general-upper-bound-thm} requires $\delta$ to decay at least as fast as $n^{-2}$. Incorporating this we get the following confidence width $\W$ and mean estimator $\hat{\mu}$,
%\begin{align*}
%    \hat{\mu}(i, u, n) = \sum_{j=1}^{u} X_j \quad \text{and} \quad \W(u, n) = f(n)\sqrt{\frac{\log(n)}{u}}
%\end{align*}
We can now obtain the cumulative regret $R_n(\pi_{\B})$ using theorem \ref{general-upper-bound-thm} and the above expression of $\W(u, n)$
\begin{corollary}
\label{bounded-regret-bound}
    \begin{align*}
        R_t(\pi_{\B}) \leq \sum_{j:\Delta_j>0} \left( 3\Delta_i + 8f(t)^2 \frac{\log(t)}{\Delta_i} \right)
    \end{align*}
\end{corollary}

We can see that the regret expression is no more logarithmic. However, the only condition on the choice of $f$ is that of being a monotonic increasing function. As a result of this, we can choose a very slow increasing function $f$ such that the regret is just a little worse than $\log(n)$. More precisely, there are several choices of $f$ for which $\pi_{\B}$ is \textit{consistent} (Definition \ref{Lattimore16.1}). Increasing functions like $c\log(t)^{\alpha}~c,a>0$, $\log(\log(t))$ are some of the possible choices of $f$. However, it is evident that slower the rate of change of $f$, higher will be the value of $t_{min}$. As an example, $t_{min} \approx 22000$ rounds if $(b-a)=10$ and $f(t)=\log(t)$.  


\begin{algorithm}[t]
  \caption{Robust Heavy RH-UCB ($\pi_{RH-UCB}$)}
  \label{robust-heavy-UCB-algo}
   \textbf{Input} $k$ arms, increasing function $f:\mathbb{N} \rightarrow \mathbb{R}$
  \begin{algorithmic}
    %\Statex \Comment { \%comment: servers[] contains the index of servers whose         data rate are sorted in descending order\%}
    %\Procedure UCB Algorithm
    %\State servers[]= index(of all servers) 
    % \State serverIndex[]=servers[0..K]
    % \State linearlyIndependentServerIndex[]=0
    % \State $[Z] \leftarrow 0$
    \State \textbf{Initialize} $\mathcal{R}_i = \{~\}$, $u_i=0$ for all arm $i$
    \State Calculate $s = \min \{t: f(t) > 0\}$
    \For  {$t=1$ to $s$}
    \State pull arm with index $i = t \mod k$ and observe reward $r$
    \State Append r to $\mathcal{R}_i$ and update $u_i \leftarrow u_i + 1$
%    \State Update $$\hat{\mu}(i, u_i, t) = \frac{1}{u_i} \sum_{X \in \mathcal{R}_i} X\mathbbm{1}_{ \left \{ |X| \leq f(t) \right \} }  $$
%    \Statex\Comment{ \%comment: find the equation corresponding the serverIndex        from the mapping at the File Server\%} 
%    \State        $eqn= equation(serverIndex[i])$ 
 %   \Statex\Comment{ \%comment: try insert equation into Z using OFG\%} 
    \EndFor 
    \For { $t=s+1, s+2, \dots$ } 
%    \Statex\Comment{\%comment: remove all the server index which were not inserted in Z\%}  
%	\State Calculate $\U(i, u, t) = \hat{\mu}(i, u, t) + \W(u, t)$
    \State Calculate the upper confidence bound as $$\U(i, u_i, t) = \underbrace{\frac{1}{u_i} \sum_{X \in \mathcal{R}_i} X\mathbbm{1}_{ \left \{ |X| \leq f(t) \right \} }}_{\hat{\mu}(i, u_i, t)} + \underbrace{\frac{1}{\log(f(t))} + f(t)\frac{8\log(t)}{u_i}}_{\W(u_i, t)} $$
	\State pull arm $i$ maximizing $\U(i, u_i, t)$ and observe reward $r$
	\State Append r to $\mathcal{R}_i$ and update $u\leftarrow u+1$
 %   \State pull $a_i = \underset{i}{\mathrm{argmin}}\text{ } \hat{\mu_{i}} + f(t) \sqrt{\frac{2\log(t)}{u_i}}$ and observe reward $r$
%    \State $\hat{\mu_t} \leftarrow \frac{\hat{\mu_t}u_i + r}{u_i + 1}$ \text{(Empirical mean update) }
%    \State $u_i \leftarrow u_i + 1$
    %temp[]=serverIndex[]-linearlyIndependentServerIndex 
    \EndFor  
    %\EndProcedure
  \end{algorithmic}
\end{algorithm}



\subsection{Confidence width $\W$, mean estimator $\hat{\mu}$ and regret $R_t(\pi_{\SG})$ for $\SG$ }
A very similar analysis is used to obtain an oblivious concentration inequality on $\{\SG\}$. In this case $t_{min} = f^{-1}(\sigma)$.
 
\begin{lemma}
\label{subgaussian-conc-inequality}
    Consider random variables $X_1, X_2, \dots, X_u \sim \SG$ with mean $\mu$. For sufficiently large $t$, with a probability less than $\delta$, we have
    \begin{align*}
        \mu - \hat{\mu} \geq f(t)\sqrt{\frac{2\log(\frac{1}{\delta})}{u}} \leq \delta \qquad \text{where} \qquad \hat{\mu} = \frac{1}{u} \sum_{j=1}^{u} X_j
    \end{align*}
\end{lemma}

%We obtain the following $\W$ and mean estimator $\hat{\mu}$ after choosing $\delta=n^{-2}$,
%\begin{align*}
%    \hat{\mu}(i, u, n) = \sum_{j=1}^{u} X_j \quad \text{and} \quad \W(u, n) = f(n)\sqrt{\frac{4\log(n)}{u}}
%\end{align*}
We again choose $\delta=t^{-4}$. The regret expression can also be obtained in similar way.
\begin{corollary}
\label{subgaussian-regret-bound}
    \begin{align*}
        R_t(\pi_{\SG}) \leq \sum_{j:\Delta_j>0} \left( 3\Delta_i + 32f(t)^2 \frac{\log(t)}{\Delta_i} \right)
    \end{align*}
\end{corollary}

%\subsection{Case 1: bounded but unknown rewards}
%
%\begin{lemma}
%\label{bounded-conc-inequality-1}
%	Consider $X_1, X_2, \dots, X_n$ be bounded random variables with mean $\mu$ such that $a<X_i<b$ for all $i$. Consider any increasing function $f$. Then, for sufficiently large $t$,
%	\begin{align*}
%		 \mathbb{P}\left(\mu - \frac{1}{n} \sum_{i=1}^{n}X_i \geq f(t) \sqrt{\frac{\log(\frac{1}{\delta})}{2n}}\right) \leq \delta
%	\end{align*}
%\end{lemma}
%%Other side of inequality
%%\mathbb{P}\left(\frac{1}{n} \sum_{i=1}^{n}X_i - \mu \geq f(t) \sqrt{\frac{\log(\frac{1}{\delta})}{2n}}\right) \leq \delta \quad \text{and} \quad

\subsection{Confidence width $\W$, mean estimator $\hat{\mu}$ and regret $R_t(\pi_{\G})$ for $\G$}

In distribution class $\{ \G \}$ we use a modified mean estimator, called the Truncated Empirical Average (TEA) estimator \ashutosh{(cite)}. Various concentration bounds have been proven with TEA \ashutosh{(cite)}, but for $\{\G(\epsilon, B)\}$. We propose a similar concentration bounds for oblivious distribution class $\{ \G \}$. In this case, we require two functions $f:\mathbb{N} \rightarrow \mathbb{R}$ and $g: \mathbb{N} \rightarrow \mathbb{R}^{+}$ to make the concentration inequality oblivious to $B$ and $\epsilon$. The constraints require $f$ to be a monotonically increasing function and $g$ to be a monotonically decreasing function while still being greater than zero for all $t$. The inequality is true for $t>\max\{t_{min}, t_{max}\}$ where $t_{min}$ is the minimum $t$ such that $f(t)\geq B$ and $t_{max}$ is the maximum $t$ such that $g(t)\leq \epsilon$. We state the inequality and then the regret upper bound as a function of number of rounds.

\begin{lemma}
\label{heavytail-conc-inequality}
    Consider random variables $X_1, X_2, \dots, X_u \sim \G$ with mean $\mu$. For sufficiently large $t$, with a probability less than $\delta$, we have
    \begin{align*}
\mu - \hat{\mu}_T \geq 4 f(t)^{\frac{1}{1+g(t)}} \left( \frac{\log(\frac{2}{\delta})}{u} \right)^{\frac{g(t)}{1+g(t)}} \quad \text{where} \quad \hat{\mu}_T = \frac{1}{u} \sum_{i=1}^{u} X_i \mathbbm{1}_{\left\{|X_i|\leq \left( \frac{uf(t)}{\log(\delta^{-1})} \right)^{\frac{1}{1+g(t)}} \right\}}
    \end{align*}
    \begin{align*}
\alternate{\mu - \hat{\mu}_T \geq \frac{1}{\log(f(t))} + f(t) \frac{\log\left( \frac{2}{\delta}\right)}{u} \quad \text{where} \quad \hat{\mu}_T = \frac{1}{u} \sum_{i=1}^{u} X_i \mathbbm{1}_{\left\{|X_i|\leq f(t) \right\}}}
    \end{align*}
\end{lemma}
We choose $\delta=t^{-4}$ to obtain width $\W$ and mean estimator $\hat{\mu}$ given in theorem \ref{general-upper-bound-thm}. Finally, we obtain the regret expression following property 2 of theorem \ref{general-upper-bound-thm}.

\begin{corollary}
\label{heavytail-regret-bound}
    \begin{align*}
        R_t(\pi_{\G_{TEA}}) \leq \sum_{j:\Delta_j>0} \left( 3\Delta_i + 8 \left( \frac{f(t)}{\Delta_i} \right) ^{\frac{1}{g(t)}} \log(2t^4) \right)
    \end{align*}
    \begin{align*}
        \alternate{R_t(\pi_{\G_{TEA}}) \leq \sum_{j:\Delta_j>0} \left( 3\Delta_i + 2\Delta_i \frac{f(t) \log\left(\frac{2}{\delta}\right)}{\Delta_i - \frac{2}{\log(f(t))}} \right) \quad \forall ~ t>t_{min}}
    \end{align*}
\end{corollary}

\alternate{We see that $t_{min}$ is the minimum $t$ for which denominator is positive, that is, $\Delta_i > \frac{2}{\log(f(t))}$. Also, we can see that the denominator increases with $t$ and asymptotically approaches $\Delta_i$. Hence, regret for $\G$ is just a little worse than $\log$ as we can choose an arbitrary slow increasing function $f(t)$. TODO: Talk about how it does not violate lower bound claimed in \citep{bubeck}}

\alternate{The following consistency argument will still be useful in the next section for MoM}

\textit{Consistency} is not immediately clear from the above regret expression. We now show that there exists appropriate choices of $f:\mathbb{N} \rightarrow \mathbb{R}$ and $g:\mathbb{N} \rightarrow \mathbb{R}^{+}$ so that the overall regret expression can be made as close to logarithmic as we want.
\begin{corollary}
\label{consistency-tea}
For every monotonic increasing function $\Phi:\mathbb{N} \rightarrow \mathbb{R}$, there exists a monotonic increasing $f:\mathbb{N} \rightarrow \mathbb{R}$, monotonic decreasing $g: \mathbb{N} \rightarrow \mathbb{R}^{+}$ and $t_1$ such that $\forall ~ \Delta_i, t>t_1$
\begin{align*}
    \left( \frac{f(t)}{\Delta_i} \right)^{\frac{1}{g(t)}} \leq \Phi(t) 
\end{align*}
\end{corollary} 
\textit{Proof:} We see that $e^{0.5(\log\Phi(t))^{1-c}}$ is an increasing function for $c \in (0, 1)$. Hence, we choose $f(t) = e^{0.5(\log\Phi(t))^{1-c}}$ and $g(t) = \frac{1}{\log^{c}(\Phi(t))}$. Also there exists $t_0$ such that for all $t>t_0$, $\frac{1}{\Delta_i} \leq e^{0.5(\log\Phi(t))^{1-c}}$ since LHS is a constant while RHS is an increasing function of $t$. Thus, we have,
\begin{align*}
    \frac{f(t)}{\Delta_i} \leq e^{(\log\Phi(t))^{1-c}}
\end{align*}
Again, there exists $t_1$ such that LHS (and hence RHS) is greater than 1. For such $t>t_1$, we have,
\begin{align*}
    \left( \frac{f(t)}{\Delta_i} \right)^{\frac{1}{g(t)}} \leq \left(e^{(\log\Phi(t))^{1-c}}\right)^{\log^{c}(\Phi(t))} = \Phi(t)
\end{align*}


%\subsection{Case 2: $\sigma$-subgaussian rewards with unknown $\sigma$}
%\begin{lemma}
%\label{subgaussian-conc-inequality}
%	Consider $X_1, X_2, \dots, X_n$ be $\sigma$-subgaussian random variables with mean $\mu$. Consider any increasing function $f$. Then, for sufficiently large $t$,
%	\begin{align*}
%		 \mathbb{P}\left(\mu - \frac{1}{n} \sum_{i=1}^{n}X_i \geq f(t) \sqrt{\frac{2\log(\frac{1}{\delta})}{n}}\right) \leq \delta
%	\end{align*}
%\end{lemma}
%%Other side
%%\mathbb{P}\left(\frac{1}{n} \sum_{i=1}^{n}X_i - \mu \geq f(t) \sqrt{\frac{2\log(\frac{1}{\delta})}{n}}\right) \leq \delta \quad \text{and} \quad
%
%\subsection{Case 3: Heavy tail assumption}
%\begin{lemma}
%\label{tea-conc-inequality}
%	Let $X_1, X_2, \dots, X_n$ be finite mean ($\mu$) random variables satisfying $\mathbb{E}[X^{1+\epsilon}] < u$. Consider an increasing function $f$ and a decreasing but positive function $g$, ($g(x)>0 \forall x$). Then, for sufficiently large $t$,
%	\begin{align*}
%		\mathbb{P}\left( \mu - \hat{\mu}_T \geq 4 f(t)^{\frac{1}{1+g(t)}} \left( \frac{\log(\frac{2}{\delta})}{n} \right)^{\frac{g(t)}{1+g(t)}} \right) \leq \delta
%	\end{align*}
%Where $\hat{\mu}_T$ is the Truncated Empirical Estimate (TEA) defined as
%\begin{align*}
%	\hat{\mu}_T = \frac{1}{n} \sum_{i=1}^{n} X_i \mathbbm{1}_{\left\{|X_i|\leq \left( \frac{un}{\log(\delta^{-1})} \right)^{\frac{1}{1+g(t)}} \right\}}
%\end{align*}
%\end{lemma}
%
%The truncation parameter used here is slightly different from the one given in \citet{bubeck} to adjust to the oblivious nature of our distributions.

\subsection{Fixed-horizon algorithm $\pi_{\G_{MoM}}$ for $\G$}
We now introduce a fixed-horizon oblivious algorithm for $\G$ with median of means as the mean estimator similar to  \citet{bubeck}, \citet{median-of-means}. Median of means estimator also assumes a weak assumption on the distribution that the central $(1+\epsilon)^{th}$ moment is finite. Similar to TEA, we use two functions 
$f:\mathbb{N} \rightarrow \mathbb{R}$ and $g: \mathbb{N} \rightarrow \mathbb{R}^{+}$ to make the concentration inequality oblivious to $\epsilon$ and the value of the upper bound on the central moment $B$. This estimator has a slightly lower $t_{min}$ since in this case, we require $f(t_{min})$ to be more than the central moment and not the absolute moment. We use a similar notation as the any-time version, except for the fact that we now use the horizon $n$ as the input to the algorithm. We replace the number of rounds $t$ with the horizon $n$ in the notation, thus $\U(i, u, n)$, $\hat{\mu}(i, u, n)$ and $\W(u, n)$ denoting the upper confidence bound, mean estimator and the confidence width. Since this is a batch algorithm, we choose one arm and pick it for $q=\floor{8\log\left(\frac{1}{\delta}\right)}$ times. We denote $v$ as the number of batches an arm has been pulled for, that is, $u=vq$. We now state a theorem similar to the any-time version.
\begin{theorem}
\label{mom-main-theorem}
Consider algorithm $\pi_{\G_{MoM}}$ We make the following choices for mean estimator $\hat{\mu}(i, u, n)$ and width $\W(u, n)$. \ashutosh{replace $\delta$ by n} 
\begin{align*}
\hat{\mu}(i, u, n) &= \text{Median}\{\hat{\mu}_1, \hat{\mu}_2, \dots, \hat{\mu}_q\} \quad \text{where} \quad \hat{\mu}_l = \frac{1}{N} \sum_{j=(l-1)N+1}^{lN} X_j\\
\W(u, n) &= (12f(n))^{\frac{1}{1+g(n)}} \left(\frac{8\log\left(\frac{1}{\delta}\right)}{u} \right)^{\frac{g(t)}{1+g(t)}}
\end{align*}
\alternate{
\begin{align*}
\W(u, n) &= f(n) \left(\frac{8\log\left(\frac{1}{\delta}\right)}{u} \right)^{g(t)}
\end{align*}
}
The following properties holds true for the algorithms:
\begin{enumerate}
    \item There exists $t_{min}$ such that for all $n>t_{min}$, $\mathbb{P}\left( |\hat{\mu}(i, u, n) - \mu_{\{i,u,n\}}| \geq \W(u, n) \right) \leq n^{-2}$
    \item $\mathbb{E}[T_i(n)] \leq u_i + 2$ where $u_i$ is the minimum $u$ satisfying $\Delta_i \geq 2\W(u, n)$
\end{enumerate}
\end{theorem}



\begin{lemma}
\label{mom-conc-inequality}
    Let $X_1, X_2, \dots, X_n$ be finite mean($\mu$) random variables satisfying $\mathbb{E}[(X-\mu)^{1+\epsilon}] < u$. Consider an increasing function $f$ and a decreasing but positive function $g$, ($g(x)>0 ~ \forall x$). Then for sufficiently large $t$,
    \begin{align*}
        \mathbb{P}\left( \hat{\mu}_M - \mu \geq (12f(t))^{\frac{1}{1+g(t)}}\left( \frac{1}{N} \right)^{\frac{g(t)}{1+g(t)}} \right) \leq \delta
    \end{align*}
    \begin{align*}
        \alternate{\mathbb{P}\left( \hat{\mu}_M - \mu \geq f(t) \left( \frac{1}{N} \right)^{g(t)} \right) \leq \delta}
    \end{align*}
where $\hat{\mu}_M$ is the Median of Means (MoM) estimator which is defined as 
\begin{align*}
    \hat{\mu}_M = \text{Median}\{\hat{\mu}_1, \hat{\mu}_2, \dots, \hat{\mu}_q\}
    \end{align*}
    \begin{align*}
    \text{where}\quad \hat{\mu}_1 = \frac{1}{N} \sum_{i=1}^{N} X_i,\quad \hat{\mu}_2 = \frac{1}{N} \sum_{i=N+1}^{2N} X_i,\quad \dots,\quad \hat{\mu}_q = \frac{1}{N} \sum_{i=(q-1)N+1}^{qN} X_i
\end{align*}
Here, $q = \floor*{8\log\left(\frac{1}{\delta}\right)}$ is the number of bins and each bin has $N = \floor*{n/q} $ samples. 
\end{lemma}

%\section{Oblivious UCB Algorithms}
%
%\begin{definition}
%	Define $\W(u, t)$ as the confidence width in the UCB algorithm, $\U(i, u, t)$ as the upper confidence bound and $\hat{\mu}(i, u, t)$ as the mean estimator. Here $i$ denote the arm index and $u$ denote the number of pulls of arm $i$ till time $t$. 
%\end{definition}
%
%\begin{theorem}
%	\label{common-regret-expression}
%	Main theorem regarding regret bound\\\\
%	\begin{tabularx}{0.9\textwidth} { 
%  | >{\raggedright\arraybackslash}X 
%  | >{\centering\arraybackslash}X
%  | >{\centering\arraybackslash}X 
%  | >{\raggedleft\arraybackslash}X | }
% \hline
% Distribution & $\W$ & $\mathbb{E}[T_i(n)]$ & $R_n$\\
% \hline
% support oblivious  & $f(t)\sqrt{\frac{\log(\frac{1}{\delta})}{2n}}$  & item 23 & item 24 \\
% \hline
% $\sigma$-oblivious  & $f(t)\sqrt{\frac{2\log(\frac{1}{\delta})}{n}}$  & item 23 & item 24 \\
% \hline
% $\epsilon, u$-oblivious (TEA)  & $4 f(t)^{\frac{1}{1+g(t)}} \left( \frac{\log(\frac{2}{\delta})}{n} \right)^{\frac{g(t)}{1+g(t)}}$  & item 23 & item 24 \\
% \hline
%\end{tabularx}
%\end{theorem}
%
%\begin{definition}
%    For the fixed budged algorithm, we define $\W(u, t)$, $\U(i, u, t)$, and $\hat{\mu}(i, u, t)$ same as above. In addition to this, denote $q$ as the batch size, and $v$ as the number of batches and hence $u=qv$. 
%\end{definition}
%
%\begin{theorem}
%\label{mom-regret-bound}
%Main theorem of MoM
%\end{theorem}


\begin{algorithm}[H]
\label{mom-main-loop}
  \caption{Fixed budget UCB Algorithm (Median of Means Estimator)}
   \textbf{Input} $k$ arms $a_1$, $a_2$, $\dots$, $a_k$, budget $T$, batch size $q$
  \begin{algorithmic}
    %\Statex \Comment { \%comment: servers[] contains the index of servers whose         data rate are sorted in descending order\%}
    %\Procedure UCB Algorithm
    %\State servers[]= index(of all servers) 
    % \State serverIndex[]=servers[0..K]
    % \State linearlyIndependentServerIndex[]=0
    % \State $[Z] \leftarrow 0$
    \State Calculate number of batches $m = \frac{T}{q}$
    \For  {$t=1$ to $k$}
    \State pull $t^{th}$ arm $q$ times and observe rewards $\{X_{i1}, X_{i2}, \dots, X_{iq}\}$
    \State Define $S_i = \{X_{i1}, X_{i2}, \dots, X_{iq}\} $ and find $\hat{\mu}(i, u, t)$ using Algorithm \ref{mom-function}
    \State Update $\W(u, t)$, and thus, $\U(i, u, t)$
%    \Statex\Comment{ \%comment: find the equation corresponding the serverIndex        from the mapping at the File Server\%} 
%    \State        $eqn= equation(serverIndex[i])$ 
 %   \Statex\Comment{ \%comment: try insert equation into Z using OFG\%} 
    \EndFor 
    \For { $t=k+1$ to $m$ } 
%    \Statex\Comment{\%comment: remove all the server index which were not inserted in Z\%}  
%	\State Calculate $\U(i, u, t)$ = $\hat{\mu}(i, u, t)$ + $\W(u, t)$
	\State pull arm $i$ minimizing $\U(i, u, t) ~ q$ times and observe rewards $\{X_{i1}, X_{i2}, \dots, X_{iq}\}$
	\State Append $\{X_{i1}, X_{i2}, \dots, X_{iq}\}$ to $S_i$ and update $\hat{\mu}(i, u, t)$ using Algorithm \ref{mom-function}
	\State Update $\W(u, t)$, and $\U(i, u, t)$
 %   \State pull $a_i = \underset{i}{\mathrm{argmin}}\text{ } \hat{\mu_{i}} + f(t) \sqrt{\frac{2\log(t)}{u_i}}$ and observe reward $r$
%    \State $\hat{\mu_t} \leftarrow \frac{\hat{\mu_t}u_i + r}{u_i + 1}$ \text{(Empirical mean update) }
%    \State $u_i \leftarrow u_i + 1$
    %temp[]=serverIndex[]-linearlyIndependentServerIndex 
    \EndFor
    %\EndProcedure
  \end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
\label{mom-function}
  \caption{Function to Calculate Median of Means (MoM)}
   \textbf{Input} $S_i = \{ X_{i1}, X_{i2}, \dots, X_{iq}, X_{i(q+1)}, \dots, X_{i(vq)} \}$ $v$ batches pulled with each having $q$ samples.
  \begin{algorithmic}
    \State Calculate $\hat{\mu}_1 = \frac{1}{v} \sum_{i=1}^{v} X_i$, $\hat{\mu}_2 = \frac{1}{v} \sum_{i=(v+1)}^{2v} X_i, \dots, \hat{\mu}_q = \frac{1}{v} \sum_{i=(q-1)v+1}^{qv} X_i $\\
    \textbf{Return} Median($\hat{\mu}_1, \hat{\mu}_2, \dots, \hat{\mu}_q$)
    %\EndProcedure
  \end{algorithmic}
\end{algorithm}
